General Graph Random Features

We propose a novel random walk-based algorithm for unbiased estimation of arbitrary functions of a weighted adjacency matrix, coined universal graph random features (u-GRFs). This includes many of the most popular examples of kernels defined on the nodes of a graph. Our algorithm enjoys subquadratic time complexity with respect to the number of nodes, overcoming the notoriously prohibitive cubic scaling of exact graph kernel evaluation. It can also be trivially distributed across machines, permitting learning on much larger networks. At the heart of the algorithm is a modulation function which upweights or downweights the contribution from different random walks depending on their lengths. We show that by parameterising it with a neural network we can obtain u-GRFs that give higher-quality kernel estimates or perform efficient, scalable kernel learning. We provide robust theoretical analysis and support our findings with experiments including pointwise estimation of fixed graph kernels, solving non-homogeneous graph ordinary differential equations, node clustering and kernel regression on triangular meshes.

==> iclr2024/old_odes.tex <==
We show now that having an unbiased estimator of the graph diffusion kernel, we can efficiently compute approximate solutions for a large class of the time-invariant non-homogeneous ordinary differential equations (ODEs) defined on graphs and consequently, conduct computations with graph kernels defined implicitly via ODE-driven graphs processes. Consider the following ODE defined on the nodes $\mathcal{N}$ of the graph $\mathcal{G}(\mathcal{N},\mathcal{E}, \mathbf{W})$:
\begin{equation}
\label{eq:ode}
\frac{d\mathbf{x}(t)}{dt} = \mathbf{W}\mathbf{x}(t) + \mathbf{Z}\mathbf{y}(t)
\end{equation}
Here $\mathbf{y}(t) \in \mathbb{R}^{N}$ defines some known process on the nodes of the graph. Furthermore, we assume that $\mathbf{Z}=\mathbf{K}_{\boldsymbol{\alpha}}(\mathbf{W})$ for some sequence $\alpha$. The solution of Eq. \ref{eq:ode} (of null boundary values) can be expressed as the convolution involving matrix exponentials:
\begin{equation}
\label{eq:x_ode}
\mathbf{x}(t) = \int_{0}^{t}\exp(\mathbf{W}(t-\tau))\mathbf{Z}\mathbf{y}(\tau)d\tau = \mathbb{E}_{\tau \sim \mathcal{P}} 
\left[\frac{1}{p(\tau)}\exp(\mathbf{W}(t-\tau))\mathbf{Z}\mathbf{y}(\tau)\right], \end{equation}
where $\mathcal{P}$ is some probabilistic distribution on the interval $[0, t]$, equipped with an efficient sampling mechanism and easy to compute pdf function $p$. We can thus unbiasedly estimate $\mathbf{x}(t)$ as follows, where $M$ is the number of Monte Carlo samples and $\tau_{1},...,\tau_{M} \overset{\mathrm{iid}}{\sim} \mathcal{P}$:
\begin{equation}
\label{eq:monte_carlo}
\widehat{\mathbf{x}}(t) = \frac{1}{M}\sum_{j=1}^{M}\frac{1}{\tau_{j}}   \exp(\mathbf{W}(t-\tau_{j}))\mathbf{Z}\mathbf{y}(\tau_{j}) 
\end{equation}
By applying uGRFs, we can now find approximate low-rank decompositions:
$\exp(\mathbf{W}(t-\tau_{j})) \approx \mathbf{A}_{j}\mathbf{B}_{j}^{\top}$ for $j=1,...,M$ as well as $\mathbf{Z} \approx \mathbf{Z}_{1}\mathbf{Z}_{2}$ for $\mathbf{A}_{j},\mathbf{B}_{j},\mathbf{Z}_{1},\mathbf{Z}_{2} \in \mathbb{R}^{N \times m}$ ($j=1,...,M$) and $m$ denoting the number of walks used to produce uGRFs. All these decompositions provide unbiased estimation of the considered matrices. Thus we can propose another unbiased estimator of $\mathbf{x}(t)$, of the following form (with brackets encoding computation order):
\begin{equation}
\label{eq:ugrf-ode}
\tilde{\mathbf{x}}(t) = \frac{1}{M}\sum_{j=1}^{M}\frac{1}{\tau_{j}}\mathbf{A}_{j}(\mathbf{B}_{j}^{\top}(\mathbf{Z}_{1}(\mathbf{Z}_{2}^{\top}\mathbf{y}(\tau_{j}))))    
\end{equation}
Note that as opposed to the standard mechanism defined by Eq. \ref{eq:monte_carlo}, 
characterized by the quadratic in the number of nodes $N$ space and time complexity,
the sampling procedure given by Eq. \ref{eq:ugrf-ode} provides linear space and time complexity for sparse graphs (since for sparse graphs uGRFs can be computed in linear time).

\paragraph{From ODEs on graphs to graph kernels:} It is easy to see that particular instantiations of Eq. \ref{eq:ode} lead to the graph diffusion process, with $\mathbf{x}(t)$ encoding graph diffusion kernel values between a given node and all the nodes of the graph, i.e. the action of the graph diffusion kernel matrix on the one-hot-vector. Equation \ref{eq:ugrf-ode} can be interpreted analogously, but for a much broader class of kernels than graph diffusion kernel.
